Efficient Action-Constrained Reinforcement Learning via Acceptance-Rejection Method and Augmented MDPs

Action-constrained reinforcement learning (ACRL) is a generic framework for learning control policies with zero action constraint violation, which is required by various safety-critical and resource-constrained applications. The existing ACRL methods can typically achieve favorable constraint satisfaction but at the cost of either high computational burden incurred by the quadratic programs (QP) or increased architectural complexity due to the use of sophisticated generative models. In this paper, we propose a generic and computationally efficient framework that can adapt a standard unconstrained RL method to ACRL through two modifications: (i) To enforce the action constraints, we leverage the classic acceptance-rejection method, where we treat the unconstrained policy as the proposal distribution and derive a modified policy with feasible actions. (ii) To improve the acceptance rate of the proposal distribution, we construct an augmented two-objective Markov decision process (MDP), which include additional self-loop state transitions and a penalty signal for the rejected actions. This augmented MDP incentives the learned policy to stay close to the feasible action sets. Through extensive experiments in both robot control and resource allocation domains, we demonstrate that the proposed framework enjoys faster training progress, better constraint satisfaction, and a lower action inference time simultaneously than the state-of-the-art ACRL methods. We have made the source code publicly available to encourage further research in this direction.

==> Algorithms/ARS_code.tex <==
\begin{algorithm}
\caption{\proposedalgorithm}
\label{al:ARS_code}
\SetAlgoNlRelativeSize{0}
\SetAlgoNlRelativeSize{-1}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Initial parameter vectors $\psi, \theta, \phi$, sample number $n$, preference sampling distribution $\mathcal{P}_{\blambda}$, number of preference vectors $N_{\blambda}$, batch size $m$, augmented ratio $\alpha$, q replay buffer update frequency $q_{f}$, actor learning rates $\xi_\pi$, critic learning rates $\xi_Q$}
Initialize real replay buffer $\mathcal{D}_{r}$\;
Initialize augmented replay buffer $\mathcal{D}_{a}$\;
\For{each iteration $j$}{
            Sample weight $\blambda$ from $\Lambda$ according $\mathcal{P}_{\blambda}$\;
    \For{each environment step $t$}{
        $k \gets 1$\;
        \While{$k \leq n$}{
            $a_t \sim \pi_{\phi}(s_t;\blambda)$\;
            \If{$a_t\in\mathcal{C}(s_t)$}
            {
              $s_{t+1} \sim \mathcal{P}(s_{t+1}|s_t, a_t)$\;
              $s_t \gets s_{t+1}$ \;
              Break\;
            }
            \Else
            {
              $k \gets k + 1$\;
              $\mathcal{D}_{a} \leftarrow \mathcal{D}_{a}  \cup \{(s_t, a_t, [0, c(s_t, a_t)], s_t)\}$\;
            }
            }
            $\tilde{a}_t \leftarrow \Pi_{\mathcal{C}(s_t)}(a_t)$\;
            Execute $\tilde{a}_t$ to obtain reward $r(s_t,\tilde{a}_t)$ from the environment\;
            
        $\mathcal{D}_{r} \leftarrow \mathcal{D}_{r}  \cup \{(s_t, a_t, [r(s_t,\tilde{a}_t), 0], s_{t+1})\}$\;
    }
    \For{each gradient step $t$}{
        Initialize update buffer $\mathcal{B}$\;
        Add $m * \alpha$ mini batches from $\mathcal{D}_{a}$ into $\mathcal{B}$\;
        Add $m - m * \alpha$ mini batches from $\mathcal{D}_{r}$ into $\mathcal{B}$\;
        Sample $N_{\blambda} - 1$  preferences and add them to set W\;
        $W \leftarrow W \bigcup \{\blambda\}$\;
        $\phi \leftarrow \phi - \xi_\pi \nabla_{\hat{\phi}} J_{\pi}(\phi)$\;
        \For{$i \in \{1, 2\}$}{
            $\theta_i \leftarrow \theta_i - \xi_Q \nabla_{\hat{\theta}_i} J_Q(\theta_i)$\;
        }
        \If{$j \% q_{f} == 0$}
        {
        $\cQ \leftarrow \cQ \cup Q_\theta$\;
        }
    }
}
\end{algorithm}


==> Algorithms/NFWPO_code.tex <==
\begin{algorithm}[H]
\caption{NFWPO Algorithm}
\label{alg:FWPO}
\DontPrintSemicolon % Removes semicolons from the end of lines in the algorithm
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Initial parameter vectors $\theta, \phi$}
\For{each iteration $t=0,1,\cdots$}{
      Select action $a_t = \pi_{\phi}(s_t) + \mathcal{N}_t$ based on current policy and exploration noise\;
    \If{$a_t$ is invalid}{
        $a_t \leftarrow \text{QP\_Solver}(s_t, a_t, \mathcal{C}(s_t))$\;
    }
  Evaluate $\pi_{\phi_{t}}$ and obtain $Q_\theta(s_t, a_t; \pi_{\phi_{t}})$\;
  \ForEach{state $s\in\mathcal{S}$}{
    Compute the Frank-Wolfe update direction by $c_{t}(s)=\arg\max_{c \in \mathcal{C}(s)}\langle c, \nabla_{a} Q_\theta(s,a;\pi_{\phi_{t}})\rangle$\;
    $g_{t}(s)=\langle c_k(s)-\pi_{\phi_{t}}(s), \nabla_{a} Q_\theta(s,a;\pi_{\phi_{t}})\rangle$\;
    $\alpha_k(s)=\frac{(1-\gamma)\mu_{\min}}{L D_s^2}g_k(s)$\;
    Update $\pi_{\phi_{t+1}}(s) \leftarrow \pi_{\phi_{t}}(s) + \alpha_k(s) (c_t(s) - \pi_{\phi_{t}}(s))$\;
  }
}
\end{algorithm}

==> Section/Sec_Exp_QP_burden.tex <==
 To highlight the burden of QP computation, we designed a more complex action-constrained experiment. We compared our algorithm with DPre+ and SPre+, proposed by \citet{kasaura2023benchmarking}, which require the QP\_Solver at each step of the update process. The testing environment is HalfCheetah, with the action constraint designed as $\Sigma_{i=1}^6 a_i^3 < 3$, which represents a 3-dimensional action constraint. Figure \ref{ex:QP_burder} presented the training curves. From this experiment, it is evident that heavily relying on a QP\_Solver during training can lead to significant inefficiencies in the overall training process.
\begin{figure}[htbp]
    \centering
        \includegraphics[width=0.5\linewidth]{Figure/halfcheetah_er_time_QP.eps}
        \caption{Training curves comparing DPre+, SPre+, and \proposedalgorithm algorithms in the HalfCheetah environment. The x-axis shows time in seconds, and the y-axis represents the average return.}
        \label{ex:QP_burder}
\end{figure}



==> bib_back_up.tex <==
% Reinforcement Learning

@article{sutton2018reinforcement,
  title={Reinforcement learning: an introduction},
  author={Sutton, Richard S},
  journal={A Bradford Book},
  year={2018}
}


% Soft Actor Critic
@inproceedings{geist2019theory,
  title={A theory of regularized markov decision processes},
  author={Geist, Matthieu and Scherrer, Bruno and Pietquin, Olivier},
  booktitle={International Conference on Machine Learning},
  pages={2160--2169},
  year={2019}
}
@inproceedings{haarnoja2017reinforcement,
  title={Reinforcement learning with deep energy-based policies},
  author={Haarnoja, Tuomas and Tang, Haoran and Abbeel, Pieter and Levine, Sergey},
  booktitle={International Conference on Machine Learning},
  pages={1352--1361},
  year={2017},
}

@inproceedings{haarnoja2018soft,
  title={{Soft actor-critic: Off-policy maximum entropy deep reinforcement learning with a stochastic actor}},
  author={Haarnoja, Tuomas and Zhou, Aurick and Abbeel, Pieter and Levine, Sergey},
  booktitle={International conference on machine learning},
  pages={1861--1870},
  year={2018},
  organization={PMLR}
}

@article{lillicrap2015continuous,
  title={Continuous control with deep reinforcement learning},
  author={Lillicrap, Timothy P and Hunt, Jonathan J and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
  journal={arXiv preprint arXiv:1509.02971},
  year={2015}
}


@inproceedings{lin2021escaping,
  title={Escaping from zero gradient: Revisiting action-constrained reinforcement learning via Frank-Wolfe policy optimization},
  author={Lin, Jyun-Li and Hung, Wei and Yang, Shang-Hsuan and Hsieh, Ping-Chun and Liu, Xi},
  booktitle={Uncertainty in Artificial Intelligence},
  pages={397--407},
  year={2021},
  organization={PMLR}
}


% ACRL
@article{kasaura2023benchmarking,
  title={Benchmarking actor-critic deep reinforcement learning algorithms for robotics control with action constraints},
  author={Kasaura, Kazumi and Miura, Shuwa and Kozuno, Tadashi and Yonetani, Ryo and Hoshino, Kenta and Hosoe, Yohei},
  journal={IEEE Robotics and Automation Letters},
  year={2023},
  publisher={IEEE}
}

% ENV
@inproceedings{todorov2012mujoco,
  title={Mujoco: A physics engine for model-based control},
  author={Todorov, Emanuel and Erez, Tom and Tassa, Yuval},
  booktitle={2012 IEEE/RSJ international conference on intelligent robots and systems},
  pages={5026--5033},
  year={2012},
  organization={IEEE}
}

@article{jay2018internet,
  title={Internet congestion control via deep reinforcement learning},
  author={Jay, Nathan and Rotman, Noga H and Godfrey, P and Schapira, Michael and Tamar, Aviv},
  journal={arXiv preprint arXiv:1810.03259},
  year={2018}
}

@inproceedings{ghosh2017incentivizing,
  title={Incentivizing the use of bike trailers for dynamic repositioning in bike sharing systems},
  author={Ghosh, Supriyo and Varakantham, Pradeep},
  booktitle={Proceedings of the International Conference on Automated Planning and Scheduling},
  volume={27},
  pages={373--381},
  year={2017}
}

@inproceedings{pham2018optlayer,
  author       = {Pham, Tu-Hoa and De Magistris, Giovanni and Tachibana, Ryuki},
  organization = {IEEE},
  booktitle    = {2018 IEEE International Conference on Robotics and Automation (ICRA)},
  date         = {2018},
  pages        = {6236--6243},
  title        = {Optlayer-practical constrained optimization for deep reinforcement learning in the real world},
}


@article{dalal2018safe,
  author = {Dalal, Gal and Dvijotham, Krishnamurthy and Vecerik, Matej and Hester, Todd and Paduraru, Cosmin and Tassa, Yuval},
  date         = {2018},
  journaltitle = {arXiv preprint arXiv:1801.08757},
  title        = {Safe exploration in continuous action spaces},
}

@article{tessler2018reward,
  title={Reward constrained policy optimization},
  author={Tessler, Chen and Mankowitz, Daniel J and Mannor, Shie},
  journal={arXiv preprint arXiv:1805.11074},
  year={2018}
}

@article{zhang2020first,
  title={First order constrained optimization in policy space},
  author={Zhang, Yiming and Vuong, Quan and Ross, Keith},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={15338--15349},
  year={2020}
}

@article{frank1956algorithm,
  title={An algorithm for quadratic programming},
  author={Frank, Marguerite and Wolfe, Philip and others},
  journal={Naval research logistics quarterly},
  volume={3},
  number={1-2},
  pages={95--110},
  year={1956},
  publisher={Wiley Subscription Services, Inc., A Wiley Company New York}
}

@article{brahmanage2024flowpg,
  title={FlowPG: Action-constrained Policy Gradient with Normalizing Flows},
  author={Brahmanage, Janaka and Ling, Jiajing and Kumar, Akshat},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{thomas2021safe,
  title={Safe reinforcement learning by imagining the near future},
  author={Thomas, Garrett and Luo, Yuping and Ma, Tengyu},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={13859--13869},
  year={2021}
}

@article{casella2004generalized,
  title={Generalized accept-reject sampling schemes},
  author={Casella, George and Robert, Christian P and Wells, Martin T},
  journal={Lecture Notes-Monograph Series},
  pages={342--347},
  year={2004},
  publisher={JSTOR}
}

@inproceedings{hung2022q,
  title={Q-Pensieve: Boosting Sample Efficiency of Multi-Objective RL Through Memory Sharing of Q-Snapshots},
  author={Hung, Wei and Huang, Bo Kai and Hsieh, Ping-Chun and Liu, Xi},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2022}
}

@article{garcia2015comprehensive,
  title={A comprehensive survey on safe reinforcement learning},
  author={Garc{\i}a, Javier and Fern{\'a}ndez, Fernando},
  journal={Journal of Machine Learning Research},
  volume={16},
  number={1},
  pages={1437--1480},
  year={2015}
}

@article{bharadhwaj2020conservative,
  title={Conservative safety critics for exploration},
  author={Bharadhwaj, Homanga and Kumar, Aviral and Rhinehart, Nicholas and Levine, Sergey and Shkurti, Florian and Garg, Animesh},
  journal={arXiv preprint arXiv:2010.14497},
  year={2020}
}

@article{thananjeyan2021recovery,
  title={Recovery rl: Safe reinforcement learning with learned recovery zones},
  author={Thananjeyan, Brijen and Balakrishna, Ashwin and Nair, Suraj and Luo, Michael and Srinivasan, Krishnan and Hwang, Minho and Gonzalez, Joseph E and Ibarz, Julian and Finn, Chelsea and Goldberg, Ken},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={3},
  pages={4915--4922},
  year={2021},
  publisher={IEEE}
}

@article{thananjeyan2020safety,
  title={Safety augmented value estimation from demonstrations (saved): Safe deep model-based rl for sparse cost robotic tasks},
  author={Thananjeyan, Brijen and Balakrishna, Ashwin and Rosolia, Ugo and Li, Felix and McAllister, Rowan and Gonzalez, Joseph E and Levine, Sergey and Borrelli, Francesco and Goldberg, Ken},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={2},
  pages={3612--3619},
  year={2020},
  publisher={IEEE}
}

@book{altman2021constrained,
  title={Constrained Markov decision processes},
  author={Altman, Eitan},
  year={2021},
  publisher={Routledge}
}

@inproceedings{achiam2017constrained,
  title={Constrained policy optimization},
  author={Achiam, Joshua and Held, David and Tamar, Aviv and Abbeel, Pieter},
  booktitle={International conference on machine learning},
  pages={22--31},
  year={2017},
  organization={PMLR}
}

@article{chen2024generative,
  title={Generative modelling of stochastic actions with arbitrary constraints in reinforcement learning},
  author={Chen, Changyu and Karunasena, Ramesha and Nguyen, Thanh and Sinha, Arunesh and Varakantham, Pradeep},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{yu2022towards,
  title={Towards safe reinforcement learning with a safety editor policy},
  author={Yu, Haonan and Xu, Wei and Zhang, Haichao},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={2608--2621},
  year={2022}
}

@inproceedings{stooke2020responsive,
  title={Responsive safety in reinforcement learning by pid lagrangian methods},
  author={Stooke, Adam and Achiam, Joshua and Abbeel, Pieter},
  booktitle={International Conference on Machine Learning},
  pages={9133--9143},
  year={2020},
  organization={PMLR}
}

@article{wen2018constrained,
  title={Constrained cross-entropy method for safe reinforcement learning},
  author={Wen, Min and Topcu, Ufuk},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}


@article{eysenbach2017leave,
  title={Leave no trace: Learning to reset for safe and autonomous reinforcement learning},
  author={Eysenbach, Benjamin and Gu, Shixiang and Ibarz, Julian and Levine, Sergey},
  journal={arXiv preprint arXiv:1711.06782},
  year={2017}
}

@inproceedings{bhatia2019resource,
  title={Resource constrained deep reinforcement learning},
  author={Bhatia, Abhinav and Varakantham, Pradeep and Kumar, Akshat},
  booktitle={Proceedings of the International Conference on Automated Planning and Scheduling},
  volume={29},
  pages={610--620},
  year={2019}
}


@article{yang2019generalized,
  title={A generalized algorithm for multi-objective reinforcement learning and policy adaptation},
  author={Yang, Runzhe and Sun, Xingyuan and Narasimhan, Karthik},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{chen2021enforcing,
  title={Enforcing policy feasibility constraints through differentiable projection for energy optimization},
  author={Chen, Bingqing and Donti, Priya L and Baker, Kyri and Kolter, J Zico and Berg{\'e}s, Mario},
  booktitle={Proceedings of the Twelfth ACM International Conference on Future Energy Systems},
  pages={199--210},
  year={2021}
}

@inproceedings{gu2017deep,
  title={Deep reinforcement learning for robotic manipulation with asynchronous off-policy updates},
  author={Gu, Shixiang and Holly, Ethan and Lillicrap, Timothy and Levine, Sergey},
  booktitle={IEEE international conference on robotics and automation},
  pages={3389--3396},
  year={2017},
  organization={IEEE}
}

@article{ichnowski2021accelerating,
  title={Accelerating quadratic optimization with reinforcement learning},
  author={Ichnowski, Jeffrey and Jain, Paras and Stellato, Bartolomeo and Banjac, Goran and Luo, Michael and Borrelli, Francesco and Gonzalez, Joseph E and Stoica, Ion and Goldberg, Ken},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={21043--21055},
  year={2021}
}

==> old_ver.tex <==
\begin{comment}
To address the Action-Constrained problem, we need to ensure that all actions during the training process satisfy the constraints. Therefore, it is necessary to perform a Quadratic Programming (QP) solver before interacting with the environment \citep{pham2018optlayer,dalal2018safe,kasaura2023benchmarking}, which requires significant computational cost. Besides, many problems have underlying action constraints that are non-convex. Due to the reliance on QP computations, the projection layer is unable to map actions onto the feasible set. In robotic control, if we cannot obtain stable actions in real-time during the implementation phase, it will lead to overall operational inefficiencies. Besides the aforementioned issues, relying heavily on a QP solver can prevent us from exploring the entire feasible set, leading to slow training. Existing methods generally fail to effectively address the aforementioned issues. A comparison with the different approaches is provided in Table \ref{tab:algorithm_comparison}. We identify that existing methods for addressing the ACRL problem often face challenges related to computational efficiency, training speed, and assumptions about the action constraint space. Therefore, there is a need for a novel method that is minimalist in both the training and testing phases while effectively addressing the ACRL problem. This work aims to propose such a method, enhancing real-time applicability and overall efficiency in action-constrained environments.
Existing methods generally fail to address these core issues, as demonstrated by the comparison in Table. Many approaches fall short in terms of computational efficiency, training speed, and assumptions about the action constraint space. As such, there is a clear need for a novel method that is minimalist in both the training and testing phases, while effectively addressing the Action-Constrained problem in reinforcement learning (ACRL).
\end{comment}
\begin{comment}
To address the Action-Constrained problem. There are already some existing Action-Constrained Reinforcement Learning (ACRL) methods. The intuitive idea is to ensure feasible actions by adding a projection layer after the policy network \citep{pham2018optlayer,dalal2018safe,kasaura2023benchmarking}. However, the projection layer requires quadratic programming operations, which are computationally expensive, especially under more complex action constraints. In robotic control, we cannot obtain stable actions in real-time during the implementation phase, leading to overall operational inefficiencies. Another method involves using additional training structures to reduce violation rates. For example, \citep{lin2021escaping} requires the Frank-Wolfe method \citep{frank1956algorithm} to find update directions, and \citep{brahmanage2024flowpg} needs extra training for flow models. These approaches increase the training burden and assume the feasible action sets are convex. A comparison with the different approaches is provided in Table \ref{tab:algorithm_comparison}. We identify that existing methods for addressing the ACRL problem often face challenges related to computational efficiency, training speed, and assumptions about the action constraint space. Therefore, there is a need for a novel method that is minimalist in both the training and testing phases while effectively addressing the ACRL problem. This work aims to propose such a method, enhancing real-time applicability and overall efficiency in action-constrained environments.
\end{comment}
\begin{comment}
To address the Action-Constrained problem. There are already some existing Action-Constrained Reinforcement Learning (ACRL) methods. The main idea is to ensure actions are feasible by adding a projection layer after the policy network \citep{pham2018optlayer,dalal2018safe}. However, this type of method will lead to the zero-gradient problem, resulting in slow training. More importantly, the projection layer requires quadratic programming operations, which are computationally expensive, especially under more complex action constraints. In robotic control, we cannot obtain stable actions in real-time during the implementation phase, leading to overall operational inefficiencies. Therefore, reducing the violation ratio of the policy network's output actions becomes a major issue. Many studies have investigated incorporating action constraints into existing deep RL algorithms. A popular approach is to apply Lagrangian Relaxation (LR) to ACRL \citep{tessler2018reward, zhang2020first}. However, defining cost signals to reduce the action violation rate effectively is difficult. Another approach is proposed in \citep{lin2021escaping}, which uses the Frank-Wolf method \citep{frank1956algorithm} to find the update direction in the feasible set. By decoupling policy gradients from the projection layer, it can effectively avoid the zero-gradient issue. However, NFWPO relies on the gradient direction for exploration, making it less effective with an imprecise critic, potentially leading to inaccurate updates and local optima. Most importantly, it requires numerous QP operations, resulting in slow training. Another approach to explore the feasible set more effectively involves training a flow model to generate action distributions that satisfy constraints and update the policy \citep{brahmanage2024flowpg}. Nonetheless, these methods require extensive data for pre-training and may not be able to train a flow model for all action constraints accurately. In summary, we believe it is important to propose a novel method that is minimalist for both training and testing while effectively addressing the ACRL problem.
\end{comment}
\begin{comment}
To address the Action-Constrained problem, we need to ensure that all actions during the training process satisfy the constraints. Hence, we require a framework that can help restrict actions to an safe range during the training process. This makes it a significant challenge to effectively train safe policies. Common approaches involve using Quadratic Programming (QP) operations \citep{pham2018optlayer,dalal2018safe,kasaura2023benchmarking} or training an additional generative model \citep{brahmanage2024flowpg}. Besides the aforementioned issues, relying heavily on a QP solver can prevent us from exploring the entire feasible set, leading to slow training. Existing methods generally fail to effectively address the aforementioned issues. A comparison with the different approaches is provided in Table \ref{tab:algorithm_comparison}. We identify that existing methods for addressing the ACRL problem often face challenges related to computational efficiency, training speed, and assumptions about the action constraint space. Therefore, there is a need for a novel method that is minimalist in both the training and testing phases while effectively addressing the ACRL problem. This work aims to propose such a method, enhancing real-time applicability and overall efficiency in action-constrained environments. 
How to achieve computationally efficient ACRL with only a minimal number of QP operations?
\end{comment}

\begin{comment}
    To address the Action-Constrained problem, it is essential to ensure that all actions during the training process satisfy the given constraints. Hence, we require a Quadratic Programming (QP) operation to restrict actions to a safe range throughout the training process. However QP is inherently complex, and its computational burden becomes significantly more severe as the dimension of the constraints increases \citep{ichnowski2021accelerating}. Therefore, reducing the reliance on QP operations becomes the primary challenge in ACRL. To overcome this challenge, we need a mechanism to sample and explore under complex constraints while reducing the action violation rate of the policy. Existing methods, such as QP-based approaches \citep{pham2018optlayer,dalal2018safe,kasaura2023benchmarking} or training an additional generative model \citep{brahmanage2023flowpg}, generally fail to effectively address these challenges. We propose a comparison of current methods in Table \ref{tab:algorithm_comparison}, and highlight their limitations in computational efficiency, training speed, and assumptions regarding the action constraint space. As such, there is a clear need for a novel method that is minimalist in both the training and testing phases. Therefore, this work primarily tackles the core question: "How can we achieve computationally efficient ACRL with only a minimal number of QP operations?"
\end{comment}
%\pch{\textbf{Solving AUTO-MDP by multi-objective RL.}  }

%With this preference, we can rewrite our objective as a linear combination $\lambda\bm{r}(s,a)$, where $\lambda$ controls the relative importance placed on the reward and penalty components. Then, we can extend the single-objective ACRL to the multi-objective setting.
 %To find the optimal policy while satisfying constraints, we present a reward penalty framework to guide the direction of updates. We establish an augmented Multi-Objective MDP (augmented MOMDP) $\tilde{\mathcal{M}} := (\mathcal{S}, \tilde{\mathcal{A}}, \tilde{\mathcal{P}}, \gamma, \tilde{\mathbf{r}}, c)$, where $\tilde{\mathcal{A}}$ represents the violated action spaces, with reward function $\tilde{\mathbf{r}}(s,a) =  \left [  0, \mathcal{K} \right ]$ where $\mathcal{K}$ is a constant penalty, and $ \tilde{\mathcal{P}}(s,a,s')$ can be redefined as follows,
%states transition back into themselves and receive the penalty when taking violated action. 
%And we define $\tilde{Q}$ as the $Q$ function for $\tilde{\mathcal{M}}$.

\begin{comment}
\begin{lemma}
Given that the lower bound and upper bound of $r(s,a)$ are $r_l$ and $r_u$, respectively, and let $\mathcal{K} < 0, r_u < 1/\gamma r_l$. 
Then, for any state $s$, if $a \in \mathcal{C}(s)$ and $a' \notin \mathcal{C}(s)$, $\blambda \tilde{Q}(s,a;\blambda)>\blambda \tilde{Q}(s,a';\blambda)$ holds, for most $\blambda \in \Lambda$
\label{lm:choose_K}
\end{lemma}
\end{comment}

\begin{comment}
\textbf{Q-Pensieve.} We know that policy updates would involve Q-snapshots from past iterations~\citep{sutton2018reinforcement}. Inspired by Envelope Q-learning~\citep{yang2019generalized}, \citet{hung2022q} proposed the Q replay buffer, designed to store snapshots of the Q-value function during the training process. By accessing the Q replay buffer, there is an opportunity to discover potentially more promising update directions for policy improvement. 
Finally, with the assistance of the Q-Pensieve, we can reformulate our objectives. Let $\phi$ and $\theta$ represent the parameters of the policy network and critic network, with $\phi^\top$ representing the parameters of the target network for the critic. 
then, we can update our policy network by minimizing the following objective, which seeks to maximize the expected reward under the current policy while incorporating the sampled preference set and Q-snapshots:

where $W(\blambda)$ denotes the preference set, which includes sampled preferences, and $\cQ$ is a set of Q-snapshots that include the current Q-value function. The overall process is summarized in the architecture shown in \cref{fg:ARS}, and the corresponding steps are detailed in \cref{al:ARS_code}, which provides a concise pseudo code for implementing the proposed method.
    
\end{comment}

\begin{comment}
\textbf{Q-Pensieve.}To improve the sampling efficiency of multi-objective reinforcement learning (MORL), \citep{hung2022q} developed a Q replay buffer, referred to as Q-Pensieve, which facilitates memory sharing across different training iterations. The Q-function influences the policy update direction. By utilizing Q-snapshots from prior training steps, Q-Pensieve potentially offers better guidance for policy improvement, leading to enhanced sampling efficiency in MORL. The Q-Pensieve approach is implemented within a policy iteration framework that alternates between two key processes in each iteration:

\begin{itemize} \item \textbf{Q-Pensieve Policy Improvement.} At each policy improvement step t, we define two sets: $W_t(\blambda)$ and $\cQ_t$. $W_t(\blambda)$ represents a collection of various preferences, including $\blambda$, and $\cQ_t$ consists of Q-snapshots from previous iterations. The policy improvement step can be reformulated as: \begin{align} \pi_{{t+1}}(\cdot\rvert \cdot;\blambda)=\arg \min_{\pi^{\prime} \in \tilde{\Pi}} \mathrm{D}_{\mathrm{KL}}\infdivx[\bigg]{\pi^{\prime}\left(\cdot \mid s;\blambda\right)}{\frac{\exp\big(\sup {\blambda' \in W_t(\blambda), \bQ^\prime \in \cQ_t}\frac{1}{\alpha} \blambda^\top \bQ^{\prime}(s, \cdot;\blambda')\big)}{Z{\cQ_t}(s)}} \label{eq: soft policy improvement} \end{align} \item \textbf{Policy Evaluation.} The policy evaluation step assesses the performance of each policy corresponding to its preference $\blambda$ by applying the multi-objective softmax Bellman operator $\mathcal{T}^{\pi}_{\text{MO}}$ iteratively, as described below: \begin{align} (\mathcal{T}^{\pi}{\text{MO}}\bQ)(s,a;\blambda)=\mathbf{r}(s,a)+\gamma\mathbb{E}_{s'\sim \mathcal{P}(\cdot|s,a),a'\sim\pi(\cdot|s';\blambda)}[\bQ(s',a';\blambda)-\alpha \log \pi(a'|s';\blambda)1_d]. \label{eq: pensieve policy evaluation} \end{align} where $\alpha$ controls the level of entropy in the system. \end{itemize}

We then integrate soft policy iteration into the MORL framework. Here, we denote the policy network parameters by $\phi$ and the critic network parameters by $\theta$. The policy update is performed by minimizing the following loss function: \begin{align} J_{\pi}(\phi) &= \sup_{\blambda' \in W(\blambda), \bQ' \in \cQ}\left[\log\pi_\phi(f_\phi(\epsilon,s;\blambda)) - \bQ'(s, f_\phi(\epsilon,s;\blambda'))\right] \label{eq:policy_update} \end{align} Subsequently, the critic network is updated by minimizing the following objective: \begin{align} J_{Q}(\theta) &= \blambda^{\top}\left(\bQ_{\theta}\left(s, a;\blambda\right)-\left({\mathbf{r}}(s,a)+\gamma \mathbb{E}{s^\prime \sim \cP(\cdot| s,a)}\left[\bQ_{\theta^\dagger}\left(s^\prime, a;\blambda\right)\right]\right)\right)^{2} \label{eq:critic_update} \end{align} where $\theta^\dagger$ represents the parameters of the target critic network. The pseudo-code for ARS can be found in Algorithm \ref{al:ARS}, and the full implementation details are provided in Algorithm \ref{al:ARS_code}.
\end{comment}

\begin{comment}
%Our algorithm is composed of three components: (i) Accept-Reject Sampling Schemes: We employ ARS~\citep{casella2004generalized} to address various action constraints. Acceptance-Rejection Sampling is a powerful method for simulating random variables from complex distributions. (ii) Augmented MOMDPs: Inspired by \citep{thomas2021safe}, we define an augmented Multi-Objective Markov Decision Process (MOMDP) apart from the original MDP for the task. In this framework, unsafe actions will cause the agent to transition back into the current state and receive a penalty. With this penalty reward scheme, we can increase the ratio that the policy outputs actions within the feasible set. However, this introduces another challenge: we need to carefully design the penalty weight to efficiently guide updates. (iii) Multi-Objective Reinforcement Learning (MORL): To balance between overall performance and the penalty weight, we reformulate the ACRL problem as a MORL problem. By leveraging the MORL framework, we can effectively train policies under varying preferences. Ultimately, by combining Augmented MOMDPs and MORL, we can significantly reduce the violation rate, thereby reducing the reliance on QP operations and achieving a lightweight solution to the ACRL problem. In the implementation, to enhance the efficiency of MORL, we combine our proposed method with the state-of-the-art MORL approach, Q-Pensieve~\citep{hung2022q}. This integration allows us to leverage Q-Pensieve’s optimization capabilities, improving the overall performance.
In this paper, we propose \proposedalgorithm and address the aforementioned issues through various architectures. First, in real-world applications, some action constraints may involve non-concave solutions. We employ Accept-Reject Sampling Schemes (ARS)~\citep{casella2004generalized} to address various action constraints. Acceptance-Rejection Sampling is a powerful method for simulating random variables from complex distributions. To encourage the agent to update towards the feasible action set, we need to design a penalty mechanism. Inspired by \citep{thomas2021safe}, we defined an augmented Multi-Objective Markov Decision Process (MOMDP) apart from the original MDP for the task. Unsafe actions will transition back into the current state and receive a penalty. This trajectory is stored separately in another replay buffer called the augmented replay buffer. During training, we will sample trajectories from both replay buffers, with the proportion of samples taken from the augmented replay buffer decaying as the training progresses. We can effectively avoid risky actions by redefining the reward as a linear combination of the original reward and penalty. Inappropriate penalties will fail to successfully train a robust and optimal policy, so determining the weights of the reward and penalty becomes a question. To overcome this issue, we can naturally consider this problem as a Multi-Objective Reinforcement Learning (MORL) problem. We can find an optimal policy that effectively reduces the action violation rate under various preferences. Therefore, we combine our proposed method with the state-of-the-art MORL approach, Q-Pensieve~\citep{hung2022q}.
\end{comment}

% % ---We propose ARS+MORL" aims to address the following issues: 1. Low sample efficiency, 2. Excessive violation, and 3. High cost.
%Our main contributions can be summarized as follows:

%\begin{itemize}
%\item We highlight that existing ACRL methods are computationally expensive to implement and propose a QP-free approach to solve ACRL problems.
%\item We revisit the ACRL algorithm through MORL to achieve good performance with a lower action violation rate.
%\item We evaluate the proposed algorithm across various domains, including locomotion and resource allocation problems. Through experimental results, we demonstrate that our method achieves better performance with lower action violation rates while also having reduced testing time during real-world interactions with the environment.
%\end{itemize}


